Discovering Latent Covariance Structures for Multiple Time Series

Analyzing multivariate time series data is important to predict future events and changes of complex systems in finance, manufacturing, and administrative decisions. The expressiveness power of Gaussian Process (GP) regression methods has been significantly improved by compositional covariance structures. In this paper, we present a new GP model which naturally handles multiple time series by placing an Indian Buffet Process (IBP) prior on the presence of shared kernels. Our selective covariance structure decomposition allows exploiting shared parameters over a set of multiple, selected time series. We also investigate the well-definedness of the models when infinite latent components are introduced. We present a pragmatic search algorithm which explores a larger structure space efficiently. Experiments conducted on five real-world data sets demonstrate that our new model outperforms existing methods in term of structure discoveries and predictive performances.

==> 3-models-old.tex <==
\subsection{\acrlong*{lgp}}

Latent GP Feature Model (gpLFM) aims to decompose $\vx_n$ into additive features in which each of them is sampled from a \acrshort*{gp}
\begin{equation}
\label{eq:decompose}
\textstyle
\vx_n = \sum_{k = 1}^K z_{nk} \vf_k + \boldsymbol{\epsilon}_n,
\end{equation}
where $z_{nk} \in \{0,1\}$ is the element of $N\times K$ matrix $\vZ$ indicating whether time series $\vx_n$ has component $\vf_k$; $\boldsymbol{\epsilon}_n$ is a vector having each element independently follows a Gaussian noise $ \mathcal{N}(0, \sigma_n^2\vI)$; for any $k = 1...K$, $\vf_{k}$ is a GP with a covariance kernel $\vC_k$, denoted as $\vf_{k} \sim \mathcal{GP}\left(\mathbf{0}, \vC_k \right).$ Here we use the GP notation for $\vf_{k}$ which is a realization of a~\acrshort*{gp}. 
% Equation~(\ref{eq:decompose}) is also referred to the linear model of corregionalization~\cite{kernel_vector}. 
When stacking $\vf_{k}$ into a $K\times D$ matrix $\vF$, our model described in (\ref{eq:decompose}) can be written as 
\begin{equation}
\textstyle
\label{eq:matrix_form}
\vX = \vZ \vF + \mathcal{E},
\end{equation}
where $\vZ$ has a finite number of rows and an unbounded number of columns. The latent features $\vf_{k}$ are shared among a set of time series $\{\vx_n|z_{nk} = 1\}$. We place the IBP prior on $\vZ$. 

Although our model represented in (\ref{eq:matrix_form}) looks similar to linear-Gaussian model in (\ref{eq:linear_gaussian}), the correlation among elements in the $k$-th row of $\vF$ described by $\vC_k$ distinguishes our model from linear-Gaussian model since there is no correlation between among elements in $\vA$. Figure \ref{fig:simple} is an illustrative explanation for~\acrshort*{lgp}.

%One may think that the IBP matrix $Z$ can be generalized to have real values like the linear model of corregionalization~\cite{kernel_vector}, or, the infinite Independent Component Analysis model~\cite{KnowlesG07_iICA}. However, this will lead to a hard model selection problem when most of all additive kernels are assigned non-zero weights. A time series will be modeled by an over-complex GP. Hence, we limit our scope on a discrete binary space for the matrix $\vZ$ where we will present structure search algorithms in Section~\ref{sec:structure_discovery}.

%%% VARIATIONAL INFERENCE %%%
\paragraph{\Acrlong*{vi} for \acrshort*{lgp}} 

We have a generative process for the data and latent variables
\begin{equation}
\label{eq:lgp}
\vZ \sim \operatorname{IBP} (\alpha),  \quad
\vf_{k}  \sim \mathcal{GP}(\mathbf{0}, \vC_k), \quad
\vx_{n}  \sim \mathcal{N}({\vz}_{n}^\top \vF, \sigma^2_n \vI),
\end{equation}

where $k \in \{1, ..., K\}$, $n\in \{1, ..., N\}$, and $\alpha$ is the concentration parameter. For simplicity, we use $\vZ \sim \operatorname{IBP} (\alpha)$ instead of explicit generative processes including (1) sample feature probabilities $\pi_{nk}$ using a Beta prior with finite case or a stick-breaking prior with infinite case; (2) then, sample $z_{nk}$ from a Bernoulli distribution parameterized by $\pi_{nk}$~\cite{vibp_Doshi}. Variational inference method approximates the true posterior $p(\vZ,\vF|\vX)$ by an variational distribution $q(\vZ,\vF)$. The method converts the optimization problem of KL divergence between $p$ and $q$ into an equivalent problem by maximizing the evidence lower bound (ELBO) $\cal L$, 
$$\textstyle \log p(\vX) =  \mathbb{E}_{\vZ, \vF}[\log p(\vX,\vZ,\vF)] + H[q] + \operatorname{KL}(q||p) \geq \mathbb{E}_{\vZ, \vF}[\log p(\vX,\vZ,\vF)] + H[q] \triangleq \mathcal{L},$$
where $\mathbb{E}$ with subscripts indicates the expectation over the approximate posterior distribution, and $H[q]$ is the entropy of $q$. The joint distribution $p(\vX,\vZ,\vF)$ is in the form of $p(\vZ)p(\vF)p(\vX|\vZ,\vF)$. We apply the mean-field variation inference, factorizing $q(\vZ, \vF) = q(\vZ)q(\vF)$. The $q(\vZ)$ is further broken down into smaller components $q(z_{nk}) = \operatorname{Bernoulli}(z_{nk};\nu_{nk})$. The distribution over the feature matrix $p(\vF)$ is written as $p(\vF) = \prod_{k=1}^K p(\vf_k)$, approximated by $q(\vF) = \prod_{k=1}^K \mathcal{N}( \vf_{k}; \vm_k, \vS_k)$. With the above specification of the variational distribution, the ELBO $\cal L$ is
$$\mathcal{L} = \expect_\vZ[\log p(\vZ)] + \expect_\vF[\log p(\vF)] + \expect_{\vZ,\vF}[\log p(\vX|\vZ,\vF)] + H[q].$$
 The detailed formula of~\acrshort*{elbo} is placed in Appendix~\ref{appendix:vi_lgp}. The~\acrshort*{lgp} differs from LFM in~\cite{vibp_Doshi} that it does not allow every element in $\vF$ freely follows an independent Gaussian noise as in LFM. Hence, in the maximization step, the variational parameters $\vm_k,\vS_k$ are updated by
 \begin{equation}
 \label{eq:phi_update}
 \textstyle
\vS_k = \left(\vC_k^{-1} + \sum_{n=1}^N\frac{\nu_{nk}}{\sigma^2_n}\vI \right)^{-1}, \quad\vm_k =\vS_k \left(\sum_{n=1}^N\frac{\nu_{nk}}{\sigma^2_n}   \left(\vx_{n} - \sum_{l:l\neq\ k} \nu_{nl}\vm_l\right) \right) .
 \end{equation}

==> 9-algorithms.tex <==
\begin{algorithm}[tbh]
\caption{Selective Search}
\label{algo}
\begin{algorithmic}[1]
%\Procedure{Search active components}{depth $d$} 
\STATE Active components $ {\mathbb{A}_1} {\leftarrow} \{{\textrm{LIN}}, {\textrm{SE}}, {\textrm{PER}}, {\textrm{C}}, {\textrm{Noise}}\}$
\STATE Seachable components $\mathbb{S}_1 \leftarrow$  A set of expanded kernels from $\mathbb{A}_{1}$
\FOR {i = 1...d}
  \FOR{$k \in \mathbb{S}_i$}
  	\STATE {Try to add $k$ to active component set $\mathbb{A}^{'}_i \leftarrow \mathbb{A}_i \cup \{k\}$}
    \STATE $Z \leftarrow$ Run VI with $\mathbb{A}^{'}_i$ 
    \IF {BIC of new model is smaller}
    	\STATE  $\mathbb{A}_i {\leftarrow} \mathbb{A}^{'}_i \backslash$\{kernel components corresponding to zero columns in  $Z$\}
    \ENDIF
  \ENDFOR
  \STATE $\mathbb{A}_{i + 1} \leftarrow \mathbb{A}_i$; $\mathbb{S}_{i + 1} \leftarrow$ A set of expanded kernels from $\mathbb{A}_{i+1}$
\ENDFOR
%\EndProcedure
\end{algorithmic}
\end{algorithm}

==> figures/tables.tex <==
\begin{table*}[tbh]
% The first row shows the results of~\cite{spike_lab}.  The second and third row are extracted from ~\cite{Hwangb16}.

\begin{minipage}[b]{0.5\linewidth}

\centering
\scalebox{0.6}{
\begin{tabular}{@{}c|ccc|ccc|c@{}}
               & 3 stocks & 6 stocks & 9 stocks & 2 houses & 4 houses & 6 houses & 4 currencies \\ \midrule \midrule
Spike and Slab & 1.80     & 2.81     & 10.26     & 13.95    & 8.59    & 11.33    & 151.37       \\
GPRN & 0.49     & 3.76     & 6.30     & 12.96    & 11.07    & 8.84    & \underbar{117.05}       \\
\acrshort*{abcd}           & 0.40      & 3.69     & 8.35     & 6.58     & 5.84     & 7.96     & 330.00       \\
\acrshort*{rabcd}          & \underbar{0.38}     & \underbar{1.22}     & \underbar{4.85}     & \underbar{2.75}     & \underbar{2.22}     & \underbar{3.10}     & 210.56       \\
\midrule
%\textit{SM}             & \textbf{0.35}     & 1.43     & \textbf{4.14}     & 5.72     & 3.13     & 4.26     & 158.17       \\
\acrshort*{lgp}    & \textbf{0.36}        & 1.47        & \textbf{4.82}      & \textbf{2.15}        & \textbf{2.08}        & \textbf{2.28}        & \textbf{81.98} \\
\acrshort*{lkm}    & \textbf{0.38}        & 1.69        & \textbf{4.30}      & \textbf{2.62}       &  2.54  
        & 3.42
                & \textbf{57.74}            
   
\end{tabular}
}
\caption{RMSEs for each data set with corresponding methods.}
\label{tab:rmse}
\end{minipage}
\hfill
\begin{minipage}[t]{0.5\linewidth}
\centering
\scalebox{1.0}{
\input{./figures/rmse_column.tex}
}
\captionof{figure}{RMSEs for each data set (9 stocks, 6 houses, 4 currencies) with corresponding methods.}
\label{fig:rmse_column}
\end{minipage}
\end{table*}
